Cross-Rollup MEV: Non-Atomic Arbitrage Across L2 Blockchains

This study quantifies the potential non-atomic MEV on Layer-2 (L2) blockchains by measuring the arbitrage opportunities between cross-rollup and DEX-CEX. Over recent years, we observe a shift in trading activities from Ethereum to rollups, with swaps on rollups occurring 2-3 times more frequently, albeit with lower trade volumes. By analyzing the costs of swap on L2s and price discrepancies cross-rollup and DEX-CEX, we identify more than 500 000 unexplored arbitrage opportunities. In particular, we find that these opportunities persist, on average, for 10 to 20 blocks, necessitating the modification of the Loss Versus Rebalancing (LVR) metric to prevent double-counting. Our findings indicate that the arbitrage opportunities in Arbitrum, Base, and Optimism range between 0.03% and 0.05% of the trading volume, while in the ZKsync it fluctuates around 0.25%.

==> sections/01x-Introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
    \label{sec:intro}
Ethereum has undergone a series of substantial enhancements aimed at increasing its functionality, addressing scalability challenges, and improving user interactions~\cite{2024EthereumRoadmap}.
%
A pivotal upgrade was the transition from \stress{Proof-of-Work~(PoW)} to \stress{Proof-of-Stake~(PoS)}, referred to as ``The Merge''---an Ethereum hard fork deployed on September~15\tsup{th},~2022~\cite{Eth-PoS,Eth-Merge}. %, which occurred throughout~2022 and~2023.
%
After that, the most significant milestone was the Dencun upgrade, implemented on March~13\tsup{th},~2024.
%
It introduced Proto-Danksharding, specifically designed for rollups: Layer-2 (L2) scaling solutions~\cite{Eth-Danksharding}.
%
This upgrade marked the initial phase of Ethereum's rollup-centric roadmap and introduced blobs, temporary storage for rollup transaction data, streamlining verification, and reducing data storage costs~\cite{2024EthereumRoadmap}. Consequently, the gas fees on rollups have been significantly reduced, as shown in Fig.~\ref{fig:rollup-fees}.

\begin{figure}[t]
\centering
    \includegraphics[width=0.95\textwidth]{figures/all-dencun.pdf} 
\caption{Median transaction fees, measured in Gwei, for selected Ethereum rollups, pre- and post-Dencun Upgrade on March~13\tsup{th},~2024.}
\label{fig:rollup-fees}
\end{figure}

The reduction in gas fees has influenced the use of Decentralized Finance (DeFi) on rollups. In recent years, the Total Value Locked (TVL) and the trading volume on rollups have exhibited a notable increase, with certain rollups now surpassing Ethereum in daily transaction numbers~\cite{2024DeFiCategories,2024L2BeatTVL}. Furthermore, the dynamics of L2 DeFi is not solely altered by reduced gas fees. The second important factor is the faster block production, typically less than~2 seconds in contrast to Ethereum's~12 seconds~\cite{Thibault2022SoKRollup}. The combination of lower gas fees and faster block production enables arbitrageurs to capitalize on smaller price discrepancies between trading venues more quickly. Although arbitrage transactions are performed predominantly on Ethereum through Maximal Extractable Value~(MEV) Boost Auctions~\cite{heimbach2024nonatomic}, an equivalent MEV boost mechanism is not present in rollups. The absence of MEV boost auctions on rollups can be explained by the fact that most rollups rely on centralized sequencers to aggregate transactions into L1 batches. 

The centralized sequencers and the associated censorship risk remain a concern within the L2 DeFi ecosystem. Additional concerns encompass transaction finality, the time period until an L2 transaction becomes irrevocable from the rollup (soft finality) or the underlying layer-1 blockchain (hard finality)~\cite{yee2022shades}. Rollups can be categorized into optimistic and Zero-Knowledge~(ZK) rollups based on transaction validity and proof mechanisms~\cite{gangwal2022survey}. Despite the seven-day hard finality period, optimistic rollups have gained user adoption more rapidly due to better Ethereum Virtual Machine (EVM) compatibility. However, ZK-rollups offer higher transaction compression, throughput, and faster hard finality, ranging from minutes to hours. The aforementioned factors~—~reduced gas fees, absence of MEV auctions, varying finality speeds, and accelerated block production~—~contribute to distinct DeFi dynamics on rollups, which warrant further investigation.

With the emergence of decentralized rollup sequencers~\cite{motepalli2023sok}, there arises a potential risk that adverse practices associated with MEV on Ethereum~\cite{qin2021quantifying} transfer to the L2 DeFi ecosystem. To address this concern, a time-boost mechanism within sequencers has been proposed~\cite{mamageishvili2023buying}. This mechanism is specifically designed to allow back-running MEVs while preventing front-running activities. 
%\mc{Is time boost really effective agains front-running? KG: Yes} 
Front-running MEV can facilitate various forms of adversarial actions, such as sandwich attacks on traders~\cite{Heimbach_2022,messias2023dissecting} and Just-In-Time (JIT) liquidity attacks on Liquidity Providers (LPs) within AMM-DEXs~\cite{zhou2021justintime}. In contrast, back-running MEV enables immediate arbitrage at DEXs or liquidations at lending protocols. Faster arbitrage execution benefits traders, as it eliminates price discrepancies between trading venues. Additionally, MEV time-boost auctions can generate new revenue for sequencer operators. 

This paper contributes to the research on L2 DeFi by empirically examining the differential swap dynamics on rollups and Ethereum, considering the factors mentioned above, such as lower gas fees, faster block production, and the absence of MEV auctions. Furthermore, we quantify the potential arbitrage opportunities across rollups and between rollups and CEXs that can be the basis for the revenue estimation from the time-boost MEV auctions in the rollup sequencers.

\parab{Related Work.} There exists a substantial body of research on DeFi, particularly focused on AMM-DEXs. In particular, the systematization of knowledge (SoK) by Xu et al.~\cite{Xu2021SoK:Protocols} and empirical investigations of Uniswap (v3) on the Ethereum blockchain~\cite{Heimbach2021BehaviorExchanges,Fritsch2021ConcentratedMakers,Heimbach2022RisksProviders,Loesch2021ImpermanentV3,gogol2024liquid} are prominent. Most of these studies evaluate the profitability of LPs, specifically addressing impermanent loss. The analysis by Adams et al.~\cite{adams2024dont} delves into the costs and dynamics of swaps on Uniswap (v3) on Ethereum. Our research extends this by breaking down swap fees on rollups and assessing the influence of blobs and block time on swap dynamics. Our findings are consistent with the simulated decomposition of swap fees in rollups presented in Gogol et al.~\cite{gogol2024crossborder}.

The Loss Versus Rebalancing metric (LVR), which compares arbitrageur profits with those of LPs, was introduced by Milionis et al.~\cite{Milionis2022AutomatedLoss-Versus-Rebalancing,milionis2023automated} and empirically measured by Fritsch et al.~\cite{fritsch2024measuring}. LVR evaluates the LP portfolio against a rebalancing portfolio that perfectly hedges the market risk of the LP position. Our investigation quantifies the absolute profit of arbitrageurs, also known as the net LVR (per block), incorporating significant adjustments. First, LVR assumes that the price discrepancies between AMMs and target exchanges, such as CEXs, disappear after each block. Our findings confirm this assumption for Uniswap (v3) on Ethereum; nonetheless, the decay period of price discrepancies on rollups extends over multiple blocks. Our methodology adjusts the LVR to this scenario and prevents double counting of the same arbitrage opportunities. Second, LVR and the rebalancing portfolio assess the LP's loss relative to arbitrageurs, thereby containing impermanent loss. Our metrics measure the absolute profit of the arbitrageur. Practically, arbitrageurs do not replicate the rebalancing portfolio but instead capitalize on arbitrage opportunities~\cite{heimbach2024nonatomic}.

The persistence of price disparities on AMMs within ZKsync Era, a ZK rollup, was initially reported by Gogol et al.~\cite{gogol2024quantifying}. Our paper builds on that research by providing:~i) a comprehensive analysis of rollups (Arbitrum, Base, Optimism, in addition to ZKsync Era) alongside Ethereum,~ii) enhanced precision in market price accuracy and per-block analysis, (improving from a 1-minute to a 1-second resolution), and~iii) an in-depth examination of Uniswap (v3), focusing on the most actively traded pools.

Heimbach et al.~\cite{heimbach2024nonatomic} focus on the estimation of arbitrage executed through MEV auctions on Ethereum, specifically addressing non-atomic arbitrage opportunities between AMMs and CEXs. Our research extends this investigation by examining rollups, where MEV auctions have not yet been implemented. Similarly, we establish the minimum threshold for arbitrage opportunities and derive the arbitrage value using AMM formulas. However, this work seeks to quantify the unexploited arbitrage, which occasionally persisted for several minutes, in contrast to the arbitrage realized via MEV on Ethereum. Other studies on arbitrage~\cite{barbon2023quality,lehar2021decentralized,berg2022empirical} focus primarily on AMM-DEX on Ethereum and/or cyclic arbitrage opportunities.

Torres et al.~\cite{torres2024rolling} is the first effort to quantify MEV in rollups. Despite the absence of MEV auctions, this research examines the heuristic for back-running arbitrage MEV, specifically focusing on swap events occurring within the same transaction in the block, within the context of cylindrical arbitrage. Our objective is to assess the potential for non-atomic arbitrage, involving CEXs, or cross-rollup price discrepancies.

Mamageishvili et al. ~\cite{mamageishvili2023buying} introduce a time boost mechanism within rollup sequencers. This mechanism facilitates back-running MEV while preventing front-running MEV. In subsequent work~\cite{mamageishvili2023shared}, a shared sequencer was proposed, enabling cross-rollup MEV auctions, such as those for arbitrage exploitation. However, these studies lack empirical quantification of arbitrage opportunities within rollups, a gap that this work seeks to address.

\parab{Contributions.}
This work contributes to the research on DeFi and MEV on L2s by quantifying the potential of non-atomic arbitrage on rollups. We conduct an empirical investigation into price disparities cross-rollups and measure the decay time. Our findings advance ongoing research on the applications of shared sequencer and time-boost (MEV) auctions. Our principal contributions are as follows.

%into the distinct swap dynamics in optimistic and ZK rollups, as compared to Ethereum, taking into account specific rollup characteristics, such as lower gas fees, faster block production, and the absence of MEV auctions. 

\point{\emph{L2 Non-atomic Arbitrage and Its Decay Time}}: 
By examining the price differences between Binancne and Uniswap (v3) WETH-USDC pools on L2s, we discover over~0.5 million unexploited arbitrage opportunities on rollups. The Maximal Arbitrage Value~(MAV) on Arbitrum, Base, and Optimism pools varies from~0.03\% to~0.05\% of trading volume, whereas in ZKsync Era, it is approximately~0.25\%. We show that price misalignment last for~10--20 blocks in rollups and present a framework to capture only one MAV during each misalignment period, avoiding the double counting of the same opportunities. The empirical MAV method, which filters out repeated arbitrage, results in five times lower arbitrage profits compared to the Loss-Versus-Rebalancing~(LVR) metric.

\point{\emph{L2 Swap Dynamics and Cost Breakdown}}: We broke down the costs of swapping on rollups and compare it to Ethereum. The analyzed WETH-USDC swap transactions on rollups occur~2--3 times more frequently than on Ethereum but are smaller in size. Furthermore, these swaps are generally not impacted by front- or back-running block slippage within the same block. Ethereum averages one WETH-USDC swap per block, while rollups have fewer swaps per block despite higher total swaps. Specifically, these swaps occur every third block on Base, fifth on Optimism, and tenth on Arbitrum. 

%We examine and break down swap fees on rollups before and after the Decun Upgrade (blobs). This allows us to gain new insights into the dynamics that shape arbitrage opportunities between DEXs and CEXs, as well as their implications for market design.

\point{\emph{Cross-Rollup MEV}}: We estimated the potential for cross-rollup MEV by analyzing the price disparities among WETH-USDC Uniswap (v3) pools on major L2s. The arbitrageurs profits are impacted by the price impact (of AMM) and, therefore, are the highest between the AMM pools with the highest token reserves.

%We conduct simulations to estimate cross-rollup arbitrage opportunities.




% \begin{itemize}
% \item \emph{Examination of Arbitrage and Swapping Costs on Rollups}: We conduct a comparative study of the costs of swapping and capturing arbitrage on rollups compared to Ethereum. Our findings indicate that, unlike Ethereum, transactions on rollups occur~2--3 times more frequently but are smaller in size. Furthermore, swaps on rollups are generally not impacted by front- or back-running block slippage typically caused by MEV. Block times impact rollup transactions; Ethereum averages one swap per block, while rollups have fewer swaps per block despite higher total swaps. Specifically, swaps occur every third block on Base, fifth on Optimism, and tenth on Arbitrum. 

% %We examine and break down swap fees on rollups before and after the Decun Upgrade (blobs). This allows us to gain new insights into the dynamics that shape arbitrage opportunities between DEXs and CEXs, as well as their implications for market design.

% \item \emph{Decay of Price Disparities}: We show that price differences last for~10--20 blocks in rollups, necessitating modifications in the empirical assessment of LVR metrics. We present a framework for empirically estimating arbitrage in cases where the decay period of price differences spans multiple blocks, capturing only the maximum arbitrage value~(MAV) during prolonged price disparities. The empirical MAV method, which filters out repeated arbitrage, indicates that LVR metrics have overestimated arbitrage by a factor of five.

% \item \emph{Estimation of Arbitrage on Rollups}: 
% By examining the price differences between Uniswap (v3) and Binance, we discovered over~0.5 million unexploited arbitrage opportunities on rollups. The MAV metric on Arbitrum, Base, and Optimism pools varies from~0.03\% to~0.05\% of trading volume, whereas in ZKsync Era, it is approximately~0.25\%, highlighting significant unresolved price differences.

% %We conduct simulations to estimate cross-rollup arbitrage opportunities.

% \end{itemize}

\parab{Paper Organization.}
Section~\ref{sec:backgound} provides an introduction to the concepts of rollups and AMMs. Section~\ref{sec:data} describes the dataset used in this study. Section~\ref{sec:price} analyzes the dynamics of swaps and breaks down their costs pre- and post-Dencun~(blobs) on Ethereum and its rollups. Section~\ref{sec:model} introduces the theory of arbitrage in AMMs and the Maximal Arbitrage Value~(MAV) framework for the empirical analysis, and section~\ref{sec:studies} presents the empirical results. Section~\ref{sec:discussion} discusses the importance of non-atomic arbitrage for rollups and future research on L2 MEV. Finally, Section~\ref{sec:conclusions} summarizes our findings and final remarks.
